Random walk diffusion simulations in semi-permeable layered media with varying diffusivity

In this paper we present analytical and random walk based solutions to diffusion in semi-permeable layered media with varying diffusivity. We propose a new random walk transit model (hybrid model) based on treating the membrane permeability and the change in diffusion as two infinitesimal separate phenomena. By conducting an extensive analytical flux analysis, the performance of our hybrid model is compared with a commonly used membrane model (reference model). We numerically demonstrate the limitations of the reference model and show the capability of our new model to overcome these restrictions. The suitability of both random walk transit models for the application to simulations of the diffusion tensor cardiovascular magnetic resonance (DT-CMR) is assessed in a histology-based domain. We consider a larger range of permeabilities to show the potential of our model to other possible applications beyond biological tissue.

==> sections/CRediT.tex <==
\section*{CRediT author statement}
% https://www.elsevier.com/authors/policies-and-guidelines/credit-author-statement

\begin{comment}
\begin{table*}[!h]
    \centering
    \caption{CRediT roles}
    \begin{tabularx}{\textwidth}{l|X}
        \textbf{Term} & \textbf{Definition} \\
        \hline
        Conceptualization & Ideas; formulation or evolution of overarching research goals and aims \\
        Methodology & Development or design of methodology; creation of models \\
        Software & Programming, software development; designing computer programs; \newline implementation of the computer code and supporting algorithms; testing of existing code components \\
        Validation & Verification, whether as a part of the activity or separate, of the overall replication/ reproducibility of results/experiments and other research outputs \\
        Formal analysis	& Application of statistical, mathematical, computational, or other formal techniques to analyze or synthesize study data \\
        Investigation & Conducting a research and investigation process, specifically performing the experiments, or data/evidence collection \\
        Resources & Provision of study materials, reagents, materials, patients, laboratory samples, animals, instrumentation, computing resources, or other analysis tools \\
        Data Curation & Management activities to annotate (produce metadata), scrub data and maintain research data (including software code, where it is necessary for interpreting the data itself) for initial use and later reuse \\
        Writing - Original Draft & Preparation, creation and/or presentation of the published work, specifically writing the initial draft (including substantive translation) \\
        Writing - Review \& Editing & Preparation, creation and/or presentation of the published work by those from the original research group, specifically critical review, commentary or revision – including pre-or postpublication stages \\
        Visualization & Preparation, creation and/or presentation of the published work, specifically visualization/data presentation \\
        Supervision & Oversight and leadership responsibility for the research activity planning and execution, including mentorship external to the core team \\
        Project administration & Management and coordination responsibility for the research activity planning and execution \\
        Funding acquisition & Acquisition of the financial support for the project leading to this publication \\
    \end{tabularx}
\end{table*}

\textbf{Conceptualization}: Jan~N.~Rose, J\'{e}r\^{o}me~Garnier-Brun ; \textbf{Formal analysis and investigation}: Jan~N.~Rose; \textbf{Writing - original draft preparation}: Jan~N.~Rose, Ignasi~Alemany ; \textbf{Writing - review and editing}: Andrew~D.~Scott, Denis~J.~Doorly; \textbf{Funding acquisition}: Andrew~D.~Scott, Denis~J.~Doorly ; \textbf{Supervision}:Andrew~D.~Scott, Denis~J.~Doorly; \textbf{Software}:Jan~N.~Rose, Ignasi~Alemany
\end{comment}



\textbf{Jan~N.~Rose}:
...,
Conceptualization,
Software,
Formal analysis,
Writing - Original Draft.
%
\textbf{Ignasi~Alemany}:
...,
Software,
Writing - Original Draft.
%
\textbf{J\'{e}r\^{o}me~Garnier-Brun}:
...,
Conceptualization.
%
\textbf{Andrew~D.~Scott}:
...,
Writing - Review \& Editing,
Supervision,
Funding Acquisition.
%
\textbf{Denis~J.~Doorly}:
...,
Writing - Review \& Editing,
Supervision,
Funding Acquisition.


==> sections/_performance_rw.tex <==
\subsubsection{Code performance}

The random walk code~\cite{SourceCode} is written in Python~3 and executes in serial, using NumPy~\cite{NumPy2020} arrays to efficiently operate on all walkers simultaneously. The parameter study in \cref{fig:rw_errorstudy} was carried out in parallel, where each unique simulation utilised a single core on a dedicated workstation with a modern Intel Xeon processor (18~cores with~\SI{2.3}{\giga\hertz}) and \SI{128}{\giga\byte}~RAM. Ignoring subtle differences between runs with different values for~$\kappa$ and~$D$, which lead to a different number of slightly more computationally-demanding barrier interactions, the runtime only depends on the time step~$\del{t}$. As seen in \cref{tab:code_perf}, the average runtime for all cases in \cref{fig:rw_errorstudy} ranges from less than one~minute for~$\del{t} = \SI{10}{\unitT}$ to almost \num{19}~hours for the smallest time step~$\del{t} = \SI{0.002}{\unitT}$. As the time step is decreased, we observe apparent hyper-linear scaling of the simulations where the runtime per time step decreases with an increase in number of steps/computations. However, this can be explained by the reduced number of overall membrane interactions at lower~$\del{t}$.

\begin{table}
    \centering
    \caption{Average simulation runtimes for different time steps~$\del{t}$ from simulations in \cref{fig:rw_errorstudy}. Each simulation used $N_p = \num{1e6}$~walkers and ran until~$t=\SI{1000}{\milli\second}$.}
    \label{tab:code_perf}
    \begin{tabularx}{0.9\textwidth}{r||C|C|C|C|C}
        Time step $\del{t}$ (\si{\unitT}) &%
        \num{0.002} & \num{0.05} & \num{1.0} & \num{10.0} \\
        \hline
        Average runtime &%
        \SI{18.59}{hrs} & \SI{104.41}{min} & \SI{390.91}{sec} & \SI{48.97}{sec} \\
    \end{tabularx}
\end{table}


==> sections/old_analytical_section.tex <==
\subsection{Analytical solution}
\label{sec:ana_problemformulation}

% describe the analytical solution


\citeauthor{Moutal2019}~\cite{Moutal2019} presented an elegant transcendental equation~$F(\lambda) \coloneqq 0$ that is to be solved in order to obtain the eigenvalues~$\lambda$ of the diffusion operator. The eigenvalues are the roots of~$F(\lambda^\star)$ where $\lambda^\star$~is an auxiliary variable considered when $F$~is evaluated on a continuous range. We offer a small modification to this below to improve behaviour in the special case of~$\lambda=0$. Then, we consider realistic, complex domains and show observed properties of~$F$ as relevant to finding the roots~$\lambda^\star_0$.

\subsubsection{Function description}

The solution assumes the time and space variables in \cref{eqn:diffusion} are separable, resulting in the ansatz
%
\begin{equation}
    U(x, t) = u(x) e^{-\lambda t} \, .
\end{equation}
%
For piecewise-constant~$D_k$, the eigenvalue problem is reduced to a Helmholtz equation
%
\begin{equation}
    D_k \, u'' + \lambda u = 0 \quad \forall x \in [b_k, b_{k+1}] \, .
    \label{eqn:Helmoltz_Di}
\end{equation}
%
Using the general solution to this ODE, which is a function of the eigenvalues, one can construct a transcendental equation ensuring that all boundary conditions are satisfied simultaneously. This is achieved through a series of matrix multiplications that link compartments together~\cite{Moutal2019}. The problem of finding eigenvalues is therefore reduced to that of finding the roots of that transcendental equation
%
\begin{equation}
\label{eqn:F(lambda)}
    F(\lambda)
    \coloneqq
    \begin{bmatrix}
        \kappa_m/\sqrt{\lambda D_{m-1}} & 1\\
    \end{bmatrix}
    %
    %\matrix{T}(\lambda)
    \matrix{R}_{m-1}(\lambda)
    \left(
    \prod_{k=0}^{m-2}{
        \matrix{M}_{k,k+1}(\lambda)
        \matrix{R}_k(\lambda)
    }
    \right)
    %
    \begin{bmatrix}
        1 \\ \kappa_0/\sqrt{\lambda D_0}
    \end{bmatrix}
    = 0
\end{equation}
%
with auxiliary matrices
%
\begin{subequations}
\begin{equation}
    \matrix{R}_k(\lambda) =
    \begin{bmatrix}
    \cos( L_k \sqrt{\lambda/D_k} ) & \sin( L_k \sqrt{\lambda/D_k} ) \\
    -\sin( L_k \sqrt{\lambda/D_k} ) & \cos( L_k \sqrt{\lambda/D_k} )
    \end{bmatrix}
    \, ,
\end{equation}
\begin{equation}
    \matrix{M}_{k,k+1}(\lambda) = 
    \begin{bmatrix}
        1 & \sqrt{\lambda D_k}/\kappa_{k,k+1} \\
        0 & \sqrt{D_k/D_{k+1}}
    \end{bmatrix}
    \, .
\end{equation}
\end{subequations}

For a sensible choice of permeabilities for internal barriers~($0 < \kappa_k < \infty$, i.e.~no trivial cases), there exist a countably infinite number of real eigenvalues, all of which are non-negative, ordered, and simple~\cite{Moutal2019}:
%
\begin{equation}
    0 \leq \lambda_{1} < \lambda_{2} < \, \dots \, , \quad \lambda_{n} \to \infty
\end{equation}
%
As shown later in \cref{sec:ana_sensitivity}, eigenvalues of higher order~$n$ have diminishing importance with increasing solution time~$t$. The truncation point is chosen based on experience and is problem-specific as seen below, for the domains in this work we use~$n \leq \order{\num{1e3}}$. Furthermore, $\lambda_1 = 0 \iff \kappa_0 = \kappa_m = 0$, which has a constant eigenmode corresponding to the steady-state solution.

\subsubsection{Computing the eigenmodes and obtaining a solution}
\label{sec:ana_solution}

While the eigenvalues~$\lambda_i$ are only dependent on the domain properties, the eigenmodes~$\nu_i(x)$ need to be evaluated at points in the domain where the solution is to be computed. We use a high number of linearly-spaced query points~$x_q \in [0, b_m]$ to discretise the domain and obtain~$\nu(x_q)$ by solving \cref{eqn:Helmoltz_Di} as done in~\cite{Moutal2019}. The time-varying solution in the domain is calculated by summation:
%
\begin{equation}
    U(x_q, t) \approx \sum_{n=1}^{N}{ e^{-\lambda_n t} \nu_n(x_q) \nu_n(x_{q,0}) }
    \label{eqn:ana_series}
\end{equation}
%
The initial condition is always given by:
%
\begin{equation}
    U(x_q, 0) = \delta(x_q - x_{q,0})
    \label{eqn:ana_initialcondition}
\end{equation}
%
As described above, the eigenvalues (roots of \cref{eqn:F(lambda)}) are found numerically up to~$\lambda_\text{max}$. The solution~$U(x_q, t)$ is, therefore, semi-analytical. As a consequence, numerical errors introduced by the root finding procedure manifest themselves as errors in the solution. Here, we attempt to quantify these errors using two approaches: comparison with a known solution and sensitivity analysis.

